Toward Low-Latency, High-Fidelity Calibration of the LIGO Detectors with Enhanced Monitoring Tools

Accurate and reliable calibration of the Advanced LIGO detectors has enabled a plethora of gravitational-wave discoveries in the detectors' first decade of operation, starting with the ground-breaking discovery, GW150914. In the first decade of operation, the calibrated strain data from Advanced LIGO detectors has become available at a lower latency and with more reliability. In this paper, we discuss the relevant history of Advanced LIGO calibration and introduce new tools that have been developed to enable faster and more robust calibrated strain data products in the fourth observing run (O4). We discuss improvements to the robustness, reliability, and accuracy of the low-latency calibration pipeline as well as the development of a new tool for monitoring the LIGO detector calibration in real time.

==> darmactuationdetails.tex <==
The modeled actuation function has evolved in complexity together with the physical system since GW150914~\cite{abbott2017calibration, cahillane2017calibration, viets2018reconstructing, sun2020characterization}.
    Let us define the actuation function for a generic stage on a generic quadruple pendulum, $a_{q,i}$, and highlight all components in gory detail, using the following equation,
    \begin{eqnarray}
    a_{q,i} & = & M_{q,i}^{D}~\textrm{exp}(-2\pi i f~\tau^{D2Q}~)~F_{q,i}^{d,DI}~ \nonumber\\
     & & \hspace{0.25in} \times \sum_{o} \bigg( M_{L2O} ~\xi_{q,i,o}^{d,O} \xi_{q,i,o}^{\textrm{d,AI}} C_{q,i,o}^{D2A}~\textrm{exp}(-2\pi i~f \tau_{q,i,o}^{D2A})~\nonumber\\
     & & \hspace{0.25in} \times \xi_{q,i,o}^{\textrm{a,AI}}~\xi_{q,i,o}^{a,LP}~ ~\kappa_{q,i,o}~h_{q,i,o}~M_{O2L} \bigg) \nonumber\\
    & &  \hspace{0.25in} \times ~S_{q,i}~M_{q,T}^{\Delta L}
    \end{eqnarray}
    with components as follows.
    From $d_{\textrm{ctrl}}$, generated from a computer process with sampling rate $f_{s}^{\textrm{(16 kHz)}}$, one choses which of the four quaduple pendula, enumerated with $q = ix, iy, ex, ey$ to drive with a $q \times i$ digital ``output'' matrix element $M_{q}^{D}$. 
    The signal is sent to the given $q$th pendula's control system computer process (synchronized by the timing system and running at the same sample rate) within one computational clock-cycle ($n_{D2Q} = 1$), and thus suffers a phase delay, $\textrm{exp}(-2\pi i~ f \tau_{D2Q})$ with $\tau_{D2Q} = 1 / f_{s}^{\textrm{(16 kHz)}}$.
    That pendula's copy of the control signal, $d_{\textrm{ctrl}}^{\textrm{q}}$, is distributed to each $i$th stage control path filtered with a dimensionless $F_{q,i}$, where $i = $U, P, T, in order to define the frequency range of use.
    For that $q^{\rm th}$ pendula's $i^{\rm th}$ stage, the filtered actuation is transformed into the basis of the physical actuators, via a digitally chosen matrix $M_{E2O}$. 
    For the lower three stages, there are four actuators per stage, each with their own electronics path, which we enumarate with $o = UL, LL, UR, LR$ (to represent their physical location, UL = upper left, LR, = lower right, etc.) and the elements of $M_{E2O}$ are merely 1/4.
    
    Once in the driver basis, each actuator's drive path contains signal conditioning electronics. 
    In reverse order these are an analog low-pass filter, $\xi_{q,i,o}^{a,LP}$, and an analog anti-imaging filter, $\xi_{q,i,o}^{a,AI}$. 
    These electronics channels are driven by a digital-to-analog converter which is running at a higher sampling rate than the control model, $f_{s}^{\textrm{(65 kHz)}}$, and thus each channel has dimension-full gain $C_{q,i,o}^{D2A}$, computational phase delay exp$(-2\pi f\tau_{q,i,o}^{D2A})$, and digital anti-aliasing filter, $\xi_{q,i,o}^{\textrm{d,AI}}$.
    The purpose of the final digital filter at $f_{s}^{\textrm(16 kHz)}$, $\xi_{q,i,o}^{d,O}$, is powerful and many fold: to (a) invert the sub-Nyquist frequency ($f_{N}^{\textrm{(16 kHz)}}$) response of each $\xi_{q,i,o}^{a,LP}$, (b) compensate the sign of the actuator if different from the intended force direction (namely magnet polarity), and (c) balance out any differential gain in the physical system, also carefully measured  with local auxiliary angular sensors, minimizing angular displacements.
    
    The resulting conditioned drive voltage or current from each actuator driver creates a frequency-independent force with dimension-full gain $h_{q,i,o}$ that may vary slowly with time, captured by the dimensionless scale factor $\kappa_{q,i,o}$.
    The force from each actuator is physically transformed into longitudinal displacement depending on their location w.r.t. the center of mass of the stage with the basis transformation matrix $M_{O2L}$, and those elements may not necessarily just be unity as the placement about the stage may not be perfectly equidistant from the center of mass.
    The dimension-full dynamical model, $S_{q,i}$ conveys how that longitudinal force on the stage center-of-mass creates longitudinal displacement of the test mass center-of-mass. 
    $S_{q,i}$ may include other non-eigenmode bending modes that also play a role in displacing the pendulum's test mass stage, T.
    Finally, $M_{q,T}^{\Delta L}$, is a signed unity coefficient that converts the longitudinal displacement of the T stage into differential arm motion.

    Great effort is put into constructing the digital filter $\xi_{q,i,o}^{d,O}$ such that we may approximate the sub-Nyquist magnitude and phase of the transfer function product for each individual chain as though it were a single longitudinal actuator with single signal chain,
    \begin{eqnarray}
        \hspace{-0.5in} \sum_{o} \bigg( M_{O2L}~\xi_{q,i,o}^{d,O} \xi_{q,i,o}^{\textrm{d,AI}} C_{q,i,o}^{D2A} \textrm{exp}(-2\pi i~f \tau_{q,i,o}^{D2A}) \xi_{q,i,o}^{\textrm{a,AI}}~\xi_{q,i,o}^{a,LP} ~\kappa_{q,i,o}~h_{q,i,o}~M_{O2L} \bigg) \nonumber\\
        \hspace{1.75in} \approx \kappa_{q,i} H_{q,i} F_{q,i}^{d,AI} F_{q,i}^{\textrm{a,AI}} F_{q,i}^{a,LP} \textrm{exp}(-2\pi i~f \tau_{q,i}^{D2A}).
    \end{eqnarray}
    Implicit in the above approximation, 
    \begin{itemize}
    \item{the dimension-full gain of common digital-to-analog converter $C_{q,i}^{D2A}$,} 
    \item{the dimensionless gain of the common analog anti-imaging filter, $F_{q,i}^{\textrm{a,AI}}$,}
    \item{the dimension-full gain of the common analog driver, $F_{q,i}^{a,LP}$,}
    \item{the static portion of the common dimension-full actuator strength, $h_{q,i}$,}
    \item{any dimensionless factors from physical realities of the basis change matrix, $M_{O2L}$, and}
    \item{the dimension-full force to displacement absolute scale of $S_{q,i}$}
    \end{itemize}
    have \emph{all} been absorbed into a dimension-full scale factor $H_{q,i}$ such that it now has units of displacement per unit of requested longitudinal control counts.
    If each quadrant's actuation strength varies independently in time, only the common mode variation will change the longitudinal actuation strength, so we set $\kappa_{q,i,o} \approx \kappa_{q,i}$.
    
    For clarity and distinction, as further simplification of our definition of $a_{q,i}$, we drop the alphabetical case of the dynamical model from dimension-full dynamical response, $S_{q,i}$, to ``just'' a dynamical frequency response, $s_{q,i}$.
    Similarly, the overall dimension-full scale is excluded from response of the analog anti-aliasing and low pass filters. 
    This leaves $F_{q,i}^{\textrm{a,AI}}$ and $F_{q,i}^{a,LP}$ representing only the frequency response of the AI filter and what super-Nyquist poles remain of the low-pass filter response after real-time compensation within each $\xi_{q,i,o}^{d,O}$. 
    A single model for all analog anti-aliasing filters is used, so $\xi_{q,i,o}^{\textrm{a,AI}} = F_{q,i}^{\textrm{a,AI}} = F^{\textrm{a,AI}}$, which is also scaled to have unity magnitude.
    The digital anti-aliasing filters (which have no scale) are programmed to be identical for all such $f_{s}^{\textrm{(16 kHz)}}$ to $f_{s}^{\textrm{(65 kHz)}}$ sampling rate exchanges, such that $\xi_{q,i,o}^{\textrm{d,AI}} = F_{q,i}^{\textrm{d,AI}} = F^{\textrm{d,AI}}$. 
    Finally, we assume that each $o$th actuator on any given stage of a given pendulum have the same computational delay, as it's at least true that those four channels are on the same DAC card. 
    So $\tau_{q,i,o}^{D2A}$ is reduced to the common $\tau_{q,i}^{D2A}$.
    
    The leaves our definition of $a_{q,i}$ dramatically simplified,
    \begin{eqnarray}
         a_{q,i} & \approx & M_{q}^{D}~\textrm{exp}(-2\pi i f \tau_{D2Q})~F_{q,i}^{d,DI}~ \nonumber\\
         & & \hspace{0.25in} \times F^{\textrm{d,AI}} ~\textrm{exp}(-2\pi i f \tau_{q,i}^{D2A})~F^{a,AI}~F_{q,i}^{a,LP}~\nonumber\\
         & & \hspace{0.25in} \times \kappa_{q,i}~H_{q,i}~s_{q,i} \nonumber\\
         & & \hspace{0.25in} \times M_{q,T}^{\Delta L}
    \end{eqnarray}
    and a slight re-arrangement to harken to previously published forms,
    \begin{eqnarray}
    a_{q,i} & \approx & \kappa_{q,i}~H_{q,i} \nonumber\\
    & & \hspace{0.25in} F_{q,i}^{d,DI} \nonumber\\
    & & \hspace{0.25in} F^{\textrm{d,AI}}~F^{a,AI}~F_{q,i}^{a,LP}~s_{q,i} \nonumber\\
    & & \hspace{0.25in} \textrm{exp}\big[-2\pi i f (\tau^{D2Q} + \tau_{q,i}^{D2A})\big] \nonumber\\
    & & \hspace{0.25in} M_{q}^{D} M_{q,T}^{\Delta L}
    \end{eqnarray}
    From here, one can mash further things together by choosing the sign of distribution matrix, $M_{q}^{D}$, to cancel that of the physical longitudinal displacement to DARM matrix $M_{q,T}^{\Delta L}$; combining the digital delays into a total delay per stage, $\tau_{q,i} = \tau_{D2Q} + \tau_{q,i}^{D2A}$, and lumping the frequency dependence that is less impactful to the response in with the suspension dynamics,
    \begin{eqnarray}
    A_{q,i} = F^{\textrm{d,AI}}~F^{a,AI}~F_{q,i}^{a,LP}~s_{q,i}.
    \end{eqnarray}
    This yields what is published as Eq. 8 in \cite{sun2020characterization}, under the condition that only one $i^{\rm th}$ stage is used,
    \begin{eqnarray}
    A^{\textrm{(model)}}_{q=1} & = & \sum_{i=U,P,T} \kappa_{q,i}~F_{q,i}^{d,DI}~H_{q,i}~A_{q,i}~\textrm{exp}(-2\pi i f \tau_{q,i}) M_{q,T}^{\Delta L} \\
     A^{\textrm{(model)}}_{O3} & = & \kappa_{U}~F_{U}~H_{U}~A_{U}~\textrm{exp}(-2\pi i f \tau_{U}) \nonumber\\
    & & \hspace{0.25in} + \kappa_{P}~F_{P}~H_{U}~A_{P}~\textrm{exp}(-2\pi i f \tau_{P}) \nonumber\\
    & & \hspace{0.25in} + \kappa_{T}~F_{T}~H_{T}~A_{T}~\textrm{exp}(-2\pi i f \tau_{T}) \label{eq:A_O3version}
    \end{eqnarray}
    where because there's only one $F$ left in \Eref{eq:A_O3version}, the superscript differenting $F_{q,i}^{d,DI}$ as a digital distribution filter is dropped. Also, because there's only one of each stage used, the $q$ is dropped from the right-hand-side.

    In \cite{abbott2017calibration}, Eq. 4 used the symbol $\mathcal{K}_{i}$ instead of $H_{i}$ to equally represent the overall scale. 
    Slow time variations $\kappa_{i}$ were left out of the definition of $A^{\textrm{(model)}}$ as they were not yet a part of the filters that produced $h_{\rm det}^{\textrm{(model)}}$ at the time. 
    Their measured values were instead incorporated into the systematic error model, $\eta_{R}^{\textrm{(model)}}$. 
    %Worse, we did not account for systematic error in the calculation of $\kappa_{i}$ themselves \cite{wade2023improving}, nor electronics component failures left small gain differences in one stage's $\xi_{q,i,o}^{a,LP}$ even after swapping for an ``identical'' driver, and updating the compensation filter $\xi_{q,i,o}^{d,O}$.
    We imposed the naive expectation that $\kappa_{U}$ and $\kappa_{P}$ did not vary in time and could be lumped together as a common multiplicative factor, $\kappa_{PU}$.
    Finally, it was assumed that each stage had the same computational delay, $\tau_{i} = \tau_{A}$.

    In the offline reproduction of $h_{\textrm{det}}^\textrm{(model)}$ -- for both O1 and O2 and the publication of \cite{cahillane2017calibration} --  the time dependence of the actuation model was parameterized with $\kappa_{\rm T}$, $\kappa_{\rm PU}$, and $\tau_A$.
    By O3, independent values for $\kappa_{i}$ and $\tau_{i}$ were measured and successfully deployed in $A^{\textrm{(model)}}$ and became part of the standard set of TDCFs.
